Smooth Quadratic Prediction Markets

When agents trade in a Duality-based Cost Function prediction market, they collectively implement the learning algorithm Follow-The-Regularized-Leader. We ask whether other learning algorithms could be used to inspire the design of prediction markets. By decomposing and modifying the Duality-based Cost Function Market Maker's (DCFMM) pricing mechanism, we propose a new prediction market, called the Smooth Quadratic Prediction Market, the incentivizes agents to collectively implement general steepest gradient descent. Relative to the DCFMM, the Smooth Quadratic Prediction Market has a better worst-case monetary loss for AD securities while preserving axiom guarantees such as the existence of instantaneous price, information incorporation, expressiveness, no arbitrage, and a form of incentive compatibility. To motivate the application of the Smooth Quadratic Prediction Market, we independently examine agents' trading behavior under two realistic constraints: bounded budgets and buy-only securities. Finally, we provide an introductory analysis of an approach to facilitate adaptive liquidity using the Smooth Quadratic Prediction Market. Our results suggest future designs where the price update rule is separate from the fee structure, yet guarantees are preserved.

==> LP.tex <==
\section{Liquidity Provisioning}

uhhh idk :)

==> adaptive_liquid_old.tex <==
\section{Adaptive Liquidity }
Inspired by the paper \textit{A General Volume-Parameterized Market Making Framework} \cite{abernethy2014general}, we adapt the framework to our setting to facilitate adaptive liquidity.
Liquidity in this context can be thought of as the sensitivity of price changes with respect to bundle purchases. 
A high liquidity would indicate that a large bundle purchase would not cause a large price change and vice-versa. 


Let $\mathbf{S} = (\reals^d )^*$ denote the history space of the market consisting of finite (and possibly empty) sequences of bundles.
We define a volume update function via an asymmetric norm. 
%The markets we consider will be defined using a cost function $N : S \times S \to \reals$, where $N(s; s')$ is the cost of purchasing the sequence $s \in S$ of bundles given the current history $s'\in S$

%%%%%%%%%%%%%%%
\begin{comment}
  \begin{definition}[Volume]
The function $V : \mathbf{S} \to \reals_{+}$ is a volume function if for all $s\in\mathbf{S}$ and $r\in\reals^d$ it satisfies
\begin{enumerate}
    \item $V(s\oplus r)\geq V(s)$
    \item  $V(s\oplus s')$ is unbounded in $|s'|$ where $s'=r\oplus r\oplus \dots \oplus r$ for some $r\neq 0$
    \item For all $s'\in S$, $V(s\oplus (\alpha r)\oplus s')$ is unbounded in $\alpha$ for $r\neq 0$. 
\end{enumerate}
\end{definition}  
\end{comment}
%%%%%%%%%%%%%%%

\begin{definition}[Asymmetric norm]
A function $g:\reals^{d}\to\reals_+$ is an asymmetric norm if it satisfies $\forall $ $x,y\in \reals^{d}$:
\begin{itemize}
    \item Non-negativity: $g(x) \geq 0$
    \item Definiteness: $g(x) = g(-x) = 0$ if and only if $x = 0$
    \item Positive homogeneity: $g(\alpha x) = \alpha g(x)$ for all $\alpha  > 0$
    \item Triangle inequality: $g(x + y) \leq g(x) + g(y)$.
\end{itemize}
\end{definition}


Recall, if $f(x)=\gamma g(x)$ for $\gamma >0$, then $f^*(y)=\gamma g^*(y/\gamma)$
We inject liquidity by scaling the conjugate function $\hat{C}$. 
Let $C^{\circ}(q;v)= \alpha (v)C(\frac{q_t}{\alpha(v)}) = \sup_{p\in \Delta_d} p \cdot q - \alpha (v)\hat{C}(p)$\rickt{Is this true, I think you can just multiply in $\alpha (v)$ into the sup? [ ]}, where $\alpha (v)$ is an increasing function called liquidity function.
As volume $v$ grows $\hat{C}$ becomes curvier (higher strong convexity), $C^{\circ}$ becomes flatter (lower smoothness), and the market \textit{enjoys} higher liquidity.
For example, with softmax, we have $C^{\circ}(q;v)=\sup_{y\in\Delta^d}\langle q,y \rangle -\alpha (v) \sum_{i=1}^{d}y_i\log y_i$ is $\alpha (v)^{-1}$ smooth via Theorem \ref{thm:dualsmoothstr}. 

%\begin{definition}
%A perspective market is a VPM  with cost function defined by
%$$C(q, v) = \alpha (v)U(q/\alpha(v)) + g(v)$$ 
%for some liquidity function $\alpha$ and profit function $g$, and cost potential $U$.
%\end{definition}

\begin{definition}[Perspective Smooth-Quadratic AD Prediction Market]
Let $g:\reals^{d}\to\reals_+$ be an asymmetric norm and define w.r.t a $s\in \mathbf{S}$ the volume update function $V(s)=\sum_{i=1}^{t}g(r_i)$.
Let $\alpha :\reals^{d}\to (0,\infty )$ be an increasing function which expresses liquidity.
Let $C$ be \textbf{CIIP} and let $C^{\circ}:\reals^{d}\times \reals_{+}\to\reals$ such that $C^{\circ}(q;v)=\alpha (v)C(\frac{q_t}{\alpha(v)})$.
Assume that $C$ is L-smooth w.r.t. $\|\cdot \|$. 
We define the cost function of a Perspective Smooth-Quadratic AD Prediction Market by 
$$ \text{Pay}_{L^{\circ}}(q_t,r_t;v_t)= \langle \nabla C^{\circ}(q_t;v_t+g(r_t)),r_t \rangle +\frac{\alpha (v_t+g(r_t))^{-1}}{2}\| r_t\|^{2}   ~.$$
\end{definition}



\begin{axiom}[Increasing liquidity (L)]
    For all $r,r'$ and all $ \epsilon >0$ there exists some $\tau $ such that if $v>\tau $ and $(q,v)$ is a valid state, then $ |N(r; q, v) - N(r; q + r', v + f(r'))| < \epsilon.$
\end{axiom}


\rick{How do we want to define this? [ ]}


\begin{axiom}[Increasing liquidity New (L)]
    For all $r,r'$ and all $ \epsilon >0$ there exists some $\tau $ such that if $v>\tau $ and $(q,v)$ is a valid state, then $ |C(r; q, v) - C(r; q + r', v + f(r'))| < \epsilon \|r\|^2.$
\end{axiom}
\begin{proof}
    Say $q_t\to q_t+r'=q_t'\to q_t'+r$ and $q_t\to q_t+r$ then 
    $$ | \langle \nabla C(q_t)-\nabla C(q_t'),q_t- (q_t+r')\rangle+\frac{L'}{2}\|r\|^2-\frac{L}{2}\|r\|^{2} |~.$$
    As $L\to 0$ (which occurs as $v\to \infty$) we get $\|\nabla C(q_t)-\nabla C(q_t')\|\leq L\|q_t-q_t'\|$ the LHS go to zero and hence $\nabla C(q_t)-\nabla C(q_t')$ goes to zero. Hence we just have the term $\frac{\|r\|^2}{2}(L'-L)$ where $|L'-L|< \epsilon'$ yet $r$ can be arbitrarily large \rick{maybe make in def of liquidity the bundle size?}
\end{proof}


\begin{axiom}[Shrinking spread (SS)]
    For all r and all $\epsilon >0$, there exists some $\tau$ such that if $v > \tau$ and $(q, v)$ is valid state, then $|N(r; q, v) + N(-r; q, v)| < \epsilon$.
\end{axiom}



\begin{theorem}
    A perspective market satisfying regularity conditions (1–5) below for some particular constants $M$, $S$, and $B$, satisfies ARB, WCL, L and SS when the following 6 conditions hold: (1) $\lim_{v\to \infty}\alpha^{'} (v)=0$;(2) $\lim_{v\to \infty}g'(v)=0$; (3) $\lim_{v\to \infty }\alpha (v)=\infty $; (4) $\lim_{v\to \infty }v\alpha '(v)/\alpha (v)^2=0$; (5) $\forall v\geq 0$, $g(v) \leq M\alpha (v)$; (6) $\forall \; v \geq  0$, $g'(v)\geq M\alpha'(v)$.
\end{theorem}

Let $\alpha (v)=v^c$ $(0 < c < 1)$ or $\log (v + 1)$, and $g(v) =M \alpha (v)$, then the conditions of the theorem all hold.

\textbf{Regulatory Conditions} \hl{I think neg-entropy $R(x)=\sum_i x_i \log x_i$ satisfies all of it}
\begin{enumerate}
    \item $R$ is a pseudo-barrier, bounded by a constant $M$ on $\Pi$.
    \item $R$ is $1/S$ strongly convex for some constant $S$, and is twice-differentiable. 
    Then $U$ is also twice-differentiable and $\nabla^2 U$ is bounded above by $S$.
    \item $R$ is closed, and therefore $R = R^{**} = U^*$
    \item $\Pi$ is bounded by a constant $B$, i.e., $\pi \in \Pi \Rightarrow \| \pi \| \leq B$.
    \item $\alpha (v)$ is a positive increasing function on $[0,\infty )$, $g(0) = 0$, and $\alpha (v)$ and $g(v)$ are continuously differentiable.
\end{enumerate}

\url{https://www.heldermann-verlag.de/jca/jca15/jca0677_b.pdf}

\rick{@Bo \cite{dudik2014market} Example 6 appears to be what we are looking for [ ]}

Homogeneous decrease in utility for information. We begin with a differentiable cost function $C$ in a
state $s$. Let $\alpha \in (0,1)$, and define $\hat{C}(q)=\alpha C(q/\alpha )$, and $\hat{s}=\alpha s$.
$\hat{C}$ is parameterized by the “liquidity parameter” $\alpha$.
The transformation $\hat{s}$ guarantees the preservation of prices, i.e., $\hat{p}(\hat{s})=\nabla \hat{C}(\hat{s})=\alpha \nabla C (\hat{s}/\alpha )\alpha = \nabla C (s)=p(s)$
We can derive that $\hat{R}(\mu )=\alpha R(\mu )$, and D˜ (µkq) =αD(µkq/α), so, for  all µ, D˜ (µks˜) = αD(µks). 
In words, the utility for all beliefs $\mu$ with respect to the current state is decreased according to the multiplier $\alpha$.

==> stochastic_gd.tex <==
\section{Stochastic GD via Smooth Quadratic AD Prediction Market}

\rick{Stochastic gradient descent expresses aggregation of beliefs. Population of agents with fixed beliefs. One agent every round gets to trade, and they maximize utility with their fixed belief. Is this stochastic gradient descent where min is population average belief?}
